CodeBERTScore: Evaluating Code Generation with Pretrained Models of Code

Since the rise of neural natural-language-to-code models (NL->Code) that can generate long expressions and statements rather than a single next-token, one of the major problems has been reliably evaluating their generated output. In this paper, we propose CodeBERTScore: an evaluation metric for code generation, which builds on BERTScore (Zhang et al., 2020). Instead of encoding only the generated tokens as in BERTScore, CodeBERTScore also encodes the natural language input preceding the generated code, thus modeling the consistency between the generated code and its given natural language context as well. We perform an extensive evaluation of CodeBERTScore across four programming languages. We find that CodeBERTScore achieves a higher correlation with human preference and with functional correctness than all existing metrics. That is, generated code that receives a higher score by CodeBERTScore is more likely to be preferred by humans, as well as to function correctly when executed. We release five language-specific pretrained models to use with our publicly available code. Our language-specific models have been downloaded more than 1,000,000 times from the Huggingface Hub. Our code and data are available at https://github.com/neulab/code-bert-score

==> conala_table_nostdev.tex <==
\centering
\begin{tabular}{lccc}
\toprule
Metric & \ktt & \pss & \spp \\
\midrule
BLEU & .374 & .604 & .543 \\
CodeBLEU & .350 & .539 & .495 \\
ROUGE-1 & .397 & .604 & .570 \\
ROUGE-2 & .429 & .629 & .588 \\
ROUGE-L & .420 & .619 & .574 \\
METEOR & .366 & .581 & .540 \\
chrF & .470 & .635 & .623 \\
CrystalBLEU & .411 & .598 & .576 \\
\midrule
\cbs & \textbf{.517} & \textbf{.674} & \textbf{.662} \\
\bottomrule
\end{tabular}
\caption{\kt{} (\ktt), \ps{} (\pss) and \spe{} (\spp) correlations with human preference. 
% The best performance is \textbf{bold}.
The reported correlation is averaged across three runs, with standard deviation shown in \Cref{tab:corr_human_appendix} due to space limitations.}
\label{tab:corr_human}

==> correlation_metrics.tex <==
\subsubsection{Correlation Metrics}\label{sec:corr_metrics}
Following best practices in natural language evalution, we used
\kt{}~(\ktt), \ps{}~(\pss) and \spe{}~(\spp) to measure the correlation between 
%\cbs{}~(\fcbs) 
each metric's scores
and the references. %~(\fref). 
% Specifically, we use human judgement $\fref_{\text{human}}$ and functional correctness $\fref_{\text{fcorr}}$ as the reference similarity functions. 
% The detailed equations can be found in Appendix \ref{sec:corr_metrics}.

\paragraph{\kt{}~(\ktt)} measures the \emph{ordinal/rank} association between a metric such as \cbs and the reference measurement. It is calculated as:
\begin{equation*}
    \tau = \frac{|\text{concordant}| - |\text{discordant}|}{|\text{concordant}| + |\text{discordant}|}
\end{equation*}
where $|\text{concordant}|$ is the number of pairs of code snippets where two measurements agree on their relative rank. That is, if $f(\hat{y_1}, y^*) > f(\hat{y_2}, y^*)$, the reference measurement also yields $\fref(\hat{y_1}, y^*) > \fref(\hat{y_2}, y^*)$.
Similarly, $|\text{discordant}|$ is the number of pairs where two measurements yield opposite ranks.
Notably, in our experiments, we restrict the code pairs to be predictions for the same question.
% the comparisons of ranks within the generations of the \emph{same} question. 

\paragraph{\ps{}~(\pss{})} 
% \pss 
measures the \emph{linear} correlation between a metric and the reference measurement. It is defined as:
\begin{equation*}
    r_p = \frac{\sum_{i=1}^N(f(\hat{y_i}, y_i^*) - \bar{f})(\fref(\hat{y_i}, y_i^*) - \bar{\fref})}{\sqrt{\sum_{i=1}^N(f(\hat{y_i}, y_i^*) - \bar{f})^2\sum_{i=1}^N(\fref(\hat{y_i}, y_i^*) - \bar{\fref})^2}}
\end{equation*}
where $N$ is the number of generations in the dataset, $\bar{f}$ is the mean \cbs of the dataset, and $\bar{\fref}$ is the mean similarity score calculated by the reference measurement.  

\paragraph{\spe{}~(\spp)}
% \spp 
measures the correlation between the \emph{ranks} produced by a metric and the reference measurement:

\begin{equation*}
    r_p = \frac{\textrm{cov}(R(f(\hat{\mathbf{Y}}), R(\fref(\mathbf{Y}^*)))}{\sigma_{R(f(\hat{\mathbf{Y}))}}
    \sigma_{R(\fref(\mathbf{Y}^{*}))}}
\end{equation*}
where $R$ returns the ranks of  code snippets in a collection of code snippets $\mathbf{Y}$. $\textrm{cov}(\cdot, \cdot)$ is the covariance of two variables and $\sigma(\cdot)$ is the standard deviation. 

==> distinguish_background.tex <==
\subsubsection{Distinguishability} We also compare different metrics using  the \emph{distinguishability} meta-metric which was proposed in the CrystalBLEU paper \citep{eghbali2022crystalbleu},
% \subsubsection{Distinguishability Metric}
% We evaluate \cbs 
% on distinguishing between code snippets with similar semantic and those have distinct semantic. 
% We leverage 
% using the distinguishability metric $d$ proposed by \citet{eghbali2022crystalbleu} which is calculated as follows:
and is computed as follows:
\begin{equation}
    d = \frac{\sum_{y_i, y_j \in \text{Pairs}_{\text{intra}}} f(y_i, y_j)}{\sum_{y_i, y_j \in \text{Pairs}_{\text{inter}}} f(y_i, y_j)}
\end{equation}\label{eq:d}
where $\text{Pair}_{\text{intra}}$ is a set of code snippet pairs from the same semantically equivalent clusters, and $\text{Pair}_{\text{inter}}$ is an equally sized set of code snippet pairs from two clusters of different functionality. Formally,
\begin{equation}
    \begin{aligned}
        &\text{Pair}_{\text{intra}} &=& \{(y_i, y_j) \mid \exists k \textrm{ such that }  y_i, y_j \in C_k\} \\
        &\text{Pair}_{\text{inter}} &=& \{(y_i, y_j) \mid \exists k \textrm{ such that } y_i \in C_k, y_j \notin C_k\}
    \end{aligned}\label{eq:distinguish}
\end{equation}
where $C_k$ is the $k$-th cluster with semantically equivalent code snippets.
%, $(C_i, c_j)$ returns the Cartesian product between set $C_i$ and set $\{c_j\}$.
Intuitively, a similarity function $f$ that can distinguish between similar and dissimilar code will produce $d$ larger than 1, meaning that code snippets from the same semantic cluster are more similar than a pair of snippets from different clusters.
% It is notable that 

\subsubsection{Dataset with Semantically Equivalent Clusters} 
%To further evaluate the performance of \cbs beyond comparing the generated code snippets with the references, 
We follow~\citet{eghbali2022crystalbleu} to evaluate whether \cbs can distinguish similar and dissimilar code mined from \share\footnote{\url{https://sharecode.io/}}, an online coding competition platform. 
Semantically equivalent code snippets are from the same coding problem, and they all pass the unit tests provided by the platform. 
The dataset consists 6958 code snippets covering 278 problems in Java and C++. 
% We use \cbs to calculate the similarity score for code pairs that share the same semantic class and code pairs that do not.
% We then measure the distinguishability of \cbs according to \Cref{eq:distinguish}.
We then computed the similarity score for code pairs that share the same semantic class and code pairs that do not, and computed the overall distinguishability score for
% intra- and inter- scores for 
BLEU, CodeBLEU, CrystalBLEU, and \cbs, according to \Cref{eq:distinguish}. 
Since the numbers of intra- and inter-class pairs grow quadratically with the number of code snippets, in our experiments we followed \citet{eghbali2022crystalbleu} to sample $N=1000$ inter- and $N=1000$ intra-class pairs. 
%The results are shown in \autoref{tab:distinct}.

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     Metric & ShareCode Java & ShareCode C++ \\
%     \midrule
%     BLEU & 2.36 & 2.51\\
%     CodeBLEU  & 1.44 & 1.42\\
%     CrystalBLEU & 5.96 & 6.94\\
%     \midrule
%     \cbs & \textbf{9.56} & \textbf{9.13}\\
%     \bottomrule
%     \end{tabular}
%     \caption{The distinguishability with different metrics as the similarity function. The best performance is \textbf{bold}.}
%     \label{tab:distinct}
% \end{table}


%Such property of \cbs is attributed to its backbone of pretrained code models.
%The masked language model loss naturally encourages similar code to have closer contextualized representation in the high-dimensional embedding space.




% We used the same dataset as \citet{eghbali2022crystalbleu}, which was collected from the ShareCode\footnote{\url{https://sharecode.io}} online coding platform, and contains solutions to programming problems. In each of Java and C++, we randomly selected 1000 pairs of examples that belong to the same problem (intra-class), and 1000 examples belonging to different problems (inter-class). 

==> dl4c/intro.tex <==
\section{Introduction}
Models of code have seen increasing accuracy 
%and performance 
% \gn{Not clear what the difference between accuracy and performance are?} 
in the past decade \citep{hindle2016naturalness,raychev2014code,alon2020structural,allamanis2018survey} for a variety of tasks such code completion \citep{fried2022incoder}, code fixing \citep{allamanis2021self,brody2020structural,berabi2021tfix}, natural-language-to-code generation \citep{yin-neubig-2017-syntactic,zhou2022doccoder} and more \citep{alon2018codeseq,alon2019code2vec}.
More recently, the rise of large language models (LLMs) of natural language 
\citep{devlin2018bert,brown2020language}
has unlocked the application of such models to code  \citep{wang2021codet5,austin2021program,chen2021evaluating}.
LLMs of code have reached such a high accuracy that they are now useful for the broad programming audience and actually save developers' time when implemented in tools such as GitHub's Copilot. 
This sharp rise in LLMs' usability was achieved thanks to their ability to accurately generate \emph{long} completions, which span multiple tokens and even lines, rather than only a single next-token as in early models \citep{allamanis2013mining,hellendoorn2017deep}.
%,nguyen2013statistical
Nevertheless, evaluating and comparing different models has remained a challenging problem \citep{xu2022systematic} that requires an accurate and reliable evaluation metric for the quality of the models' generated outputs, and existing metrics are sub-optimal.


\input{dl4c/intro_code_example.tex}

\paragraph{Existing Evaluation Approaches}
The most common evaluation metrics are token-matching methods such as BLEU \citep{papineni2002bleu}, adopted from natural language processing. These metrics are based on counting overlapping n-grams in the generated code and the reference code.
CrystalBLEU \citep{eghbali2022crystalbleu} has recently extended BLEU by ignoring the  500 most occurring n-grams, arguing that they are trivially shared between the prediction and the reference. Nonetheless, both BLEU and CrystalBLEU rely on the lexical \emph{exact match} of tokens, which does not account for diversity in implementation, variable names, and code conventions. \Cref{fig:intro_example} shows an example: given the reference code in \Cref{subfig:reference}, both BLEU and CrystalBLEU prefer (rank higher) \emph{the non-equivalent} code in \Cref{subfig:noneq} over the functionally equivalent code in \Cref{subfig:eq}.

CodeBLEU \citep{ren2020codebleu} attempts to lower the requirement for lexical exact match, by relying on data-flow and Abstract Syntax Tree (AST) matching as well; nevertheless,  valid generations may have different ASTs and data-flow from the reference code, which may lead to low CodeBLEU score even when the prediction is correct. Further, \emph{partial} predictions may be useful for a programmer,
%(for example, predicting the first line of a \texttt{for} loop, without the loop's body and closing), 
but accepting them may lead to partial code that does not parse, and thus cannot be fully evaluated by CodeBLEU.
%
Execution-based evaluation attempts to address these problems by running tests on the generated code to verify its functional correctness \citep{chen2021evaluating,athiwaratkun2022multi,li2022competition,wang2022execution,lai2022ds}. This provides a direct measure of the functionality of the generated code, while being agnostic to diversity in implementation and style. However, execution-based evaluation requires datasets that are provided with hand-written test cases for each example, which is costly and labor-intensive to create; thus, only few such datasets exist. Further, executing model-generated code is susceptible to security threats,\footnote{\url{https://twitter.com/ludwig_stumpp/status/1619701277419794435?s=46&t=5vlJ05ph9UuGxQc17TXcrA}} and thus should be run in an isolated sandbox, which makes it technically cumbersome to work with.


\paragraph{Our Approach}
In this work, we introduce \cbs, an evaluation metric for code generation, leveraging pretrained models such as CodeBERT \citep{feng2020codebert}, and adopting best practices from natural language generation evaluation \citep{zhangbertscore}.
First, \cbs encodes the generated code and the reference code independently with pretrained models, \emph{with} the inclusion of natural language context if available.
Then, we compute the dot-product similarity between the encoded representations of each token in the generated code and the reference code. Finally, the best matching token vector pairs are used to compute precision and recall.
%\cbs$_{\mathrm{Precision}}$ and \cbs$_{\mathrm{Recall}}$
%precision and recall. 
\cbs allows comparing code pairs that are lexically different, while taking into account the (1) natural language context, if such provided; the (2) contextual information of each token; %as encoded by the BERT-based model; 
and (3) implementation diversity. %, for example by giving a high similarity score to the encoding of \texttt{for} and the encoding of \texttt{while}. 
Our approach is illustrated in \Cref{fig:mainfigure}.

\paragraph{Example}
A concrete example is shown in \Cref{fig:intro_example}: 
%, 
while BLEU and CodeBLEU prefer
% (rank higher) 
\emph{the non-equivalent} code in \Cref{subfig:noneq} given the reference code in \Cref{subfig:reference}, \cbs prefers the code in \Cref{subfig:eq}, which \emph{is} functionally equivalent to the reference. %, even though all variable names are identical across \Cref{fig:intro_example}, which helps lexical-matching methods such as BLEU. 
% We note that in this example, the variable names are identical across three code snippets. If the variable names of the reference are different than the candidate's, it is even harder for token-matching approaches such as BLEU and CrystalBLEU to compare the reference with the candidates, while \cbs can trivially match variable names according to their semantic similarity and their functional role in the code.
% Our approach is demonstrated in \Cref{fig:mainfigure}.






\paragraph{Contributions} In summary, our main contributions are:
\begin{inparaenum}[(a)]
    % \item The recognition of the absence of a reliable and static evaluation metric for code generation;
    \item a new metric for code similarity, adopted from natural language processing (NLP), which leverages the benefits of pretrained models, while not requiring manual labeling or annotation;    
    \item an extensive evaluation across four programming languages, showing that \cbs is more correlated with human preference \emph{and} more correlated with execution correctness than all previous approaches including BLEU, CodeBLEU, and CrystalBLEU;
    \item we pretrain and release five language-specific CodeBERT models to use with our publicly available code, for Java, Python, C, C++, and JavaScript. As of the time of this submission, our models have been downloaded from the Huggingface Hub more than \textbf{\downloaded} times.
\end{inparaenum}
% \gn{I'm not sure if the following is important enough to be in the intro?}
% Finally, while \cbs also achieves a higher ``distinguishability''  than CrystalBLEU, which proposed this meta-metric, we show that distinguishability can be easily manipulated and we can craft a variant of \cbs  that  achieves as high distinguishability as we wish. 
%by simply exponentiating every output score. 
% We thus suggest that distinguishability is not a reliable meta-metric in its current form, contrasting the findings of \citet{eghbali2022crystalbleu}.

\input{dl4c/intro_figure.tex}

==> dl4c/intro_code_example.tex <==
\newcommand{\lsize}{0.4\textwidth}
\newcommand{\msize}{0.45\textwidth}
\newcommand{\rsize}{0.51\textwidth}

\begin{figure*}[t]
\centering
\begin{minipage}{\lsize}
\centering
\textbf{Reference:} 
% Reference:
\end{minipage}\\
\begin{minipage}{\lsize}
\begin{minted}[fontsize=\scriptsize,stripnl=false,framesep=1pt,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
int f(Object target) {
  int i = 0;
  for (Object elem: this.elements) {
    if (elem.equals(target)) {
      return i;
    }
    i++;
  }
  return -1;
}
\end{minted}
\end{minipage} \\
\begin{minipage}{0.8\textwidth}
  \centering
  \begin{subfigure}[b]{1\linewidth}
  % \vspace{2mm}
  \caption{The ground truth reference -- find \emph{the index} of \texttt{target} in \texttt{this.elements}.}
  % \caption{\phantom{\large{\textbf{Reference:} }}}
  \label{subfig:reference}
  \end{subfigure}
  \end{minipage} \\
\begin{minipage}{\msize}
  \centering
  \textbf{Non-equivalent candidate:} 
  % Non-equivalent implementation:
  \end{minipage} 
  \hfill
  \begin{minipage}{\rsize}
  \centering
  \textbf{Equivalent candidate:} 
  % Equivalent implementation:
  \end{minipage} \\
\begin{minipage}{\msize}
\begin{minted}[fontsize=\scriptsize,stripnl=false,framesep=1pt,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
boolean f(Object target) {
  for (Object elem: this.elements) {
    if (elem.equals(target)) {
      return true;
    }
  }
  
  return false;
}


\end{minted}
\end{minipage}
\hfill
\begin{minipage}{\rsize}
\begin{minted}[fontsize=\scriptsize,framesep=1pt,stripnl=false,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
int f(Object target) {
  for (int i=0; i<this.elements.size(); i++) {
    Object elem = this.elements.get(i);
    if (elem.equals(target)) {
      return i;
    }
  }
  return -1;
}

\end{minted}
\end{minipage}

\begin{minipage}{\msize}
\centering
\begin{subfigure}[b]{1\linewidth}
\caption{\textbf{\textcolor{red}{Preferred by BLEU \& CrystalBLEU}}  -- find \emph{whether or not} \texttt{target} is in \texttt{this.elements}.}
\label{subfig:noneq}
\end{subfigure}
\end{minipage}
\hfill
\begin{minipage}{\rsize}
\centering
\begin{subfigure}[b]{1\linewidth}
\centering
\caption{\textbf{\textcolor{ForestGreen}{Preferred by \cbs}}  -- find \emph{the index} of \texttt{target} in \texttt{this.elements}.}
\label{subfig:eq}
\end{subfigure}
\end{minipage}
\caption{An intuitive example for the usefulness of \cbs in measuring generated code: \Cref{subfig:reference} shows a reference code snippet in Java. This reference can be the ground truth code given as part of a test set. \Cref{subfig:noneq} and \Cref{subfig:eq} show two generated predictions.
%, with the main difference that \Cref{subfig:noneq} \emph{is not} functionally equivalent to the reference, while \Cref{subfig:eq} \emph{is} functionally equivalent to the reference. 
Among these two candidates and given the reference, both BLEU \citep{papineni2002bleu} and CrystalBLEU \citep{eghbali2022crystalbleu} prefer (score higher) the snippet in \Cref{subfig:noneq}, which \emph{is not} functionally equivalent to the reference, while our proposed \cbs prefers the code in \Cref{subfig:eq}, which \emph{is} functionally equivalent to the code in \Cref{subfig:reference}. 
}
\label{fig:intro_example}
\end{figure*}

==> dl4c/intro_figure.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{icse/codebertscore-py.pdf}
\caption{A diagram illustrating \cbs: We use a language-specific CodeBERT model to encode each of $\langle$\emph{natural\_language}, \emph{reference\_code}$\rangle$ and $\langle$\emph{natural\_language}, \emph{generated\_code}$\rangle$. We then compute the pairwise cosine similarity between every encoded token in the reference and every encoded token in the generated code, ignoring the encoded natural language context tokens and encoded punctuation tokens; finally, we take the $max$ across the rows of the resulting matrix to compute \emph{Precision} (\textmd{\texttt{np.mean(np.max(similarity\_matrix, axis=0))}}), and across columns to compute \emph{Recall} (\textmd{\texttt{np.mean(np.max(similarity\_matrix, axis=1))}}).
}
\label{fig:mainfigure}
\end{figure*}

==> fse/commands.tex <==
\newcommand{\pair}{code-explanation\xspace}
\newcommand{\ours}{\textsc{CodeBertScore}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\todo}[1]{\textcolor{red}{TODO: #1}}
\newcommand{\sz}[1]{\textcolor{blue}{#1 -SZ}}
\newcommand{\sent}[1]{``\textit{#1}''}
\newcommand{\fbseries}{\unskip\setBold\aftergroup\unsetBold\aftergroup\ignorespaces}
\newcommand{\inlineCode}[1]{\xspace\texttt{\fbseries #1}}
\newcommand{\mask}{\texttt{[MASK]}\xspace}
\newcommand{\maski}[1]{\texttt{[MASK:#1]}\xspace}
\newcommand{\token}[1]{\texttt{[#1]}\xspace}
\newcommand{\rmark}{\ding{51}\xspace}
\newcommand{\cmark}{$\clubsuit$\xspace}
\newcommand{\xmark}{$\spadesuit$\xspace}
\newcommand{\he}{HumanEval\xspace}
\newcommand{\conala}{CoNaLa\xspace}
\newcommand{\share}{ShareCode\xspace}
\newcommand{\davinci}{\texttt{code-davinci-002}\xspace}
\newcommand{\kt}{Kendall-Tau\xspace}
\newcommand{\ps}{Pearson\xspace}
\newcommand{\spe}{Spearman\xspace}
\newcommand{\ktt}{\ensuremath{\tau}\xspace}
\newcommand{\pss}{\ensuremath{r_p}\xspace}
\newcommand{\spp}{\ensuremath{r_s}\xspace}
\newcommand{\fs}{\ensuremath{f(c_1, c_2)}}
\newcommand{\fcbs}{\ensuremath{f_{\text{cbs}}}}
\newcommand{\fref}{\ensuremath{f^*}}

==> fse/intro.tex <==
\input{dl4c/intro_code_example.tex}
\section{Introduction}
Models of code have seen increasing accuracy and performance in the past decade \citep{hindle2016naturalness,raychev2014code,alon2020structural,allamanis2018survey} for a variety of tasks such code completion \citep{fried2022incoder}, code fixing \citep{brody2020structural,berabi2021tfix,bader2019getafix}, natural-language-to-code generation \citep{yin-neubig-2017-syntactic,zhou2022doccoder} and more \citep{mastropaolo2021studying,alon2018codeseq,alon2019code2vec}.
More recently, the rise of large language models (LLMs) of natural language 
\citep{devlin2018bert,radfordimproving,brown2020language}
has unlocked the application of such models to code  \citep{wang2021codet5,xu2022systematic,austin2021program,chen2021evaluating}.
LLMs of code have reached such a high accuracy, which made them useful for the broad programming audience and actually save developers' time when implemented in tools such as GitHub's Copilot. 
This sharp rise in LLMs' usability was achieved thanks to their ability to accurately generate \emph{long} completions, which span multiple tokens and even lines, rather than only a single next-token as in early models \citep{allamanis2013mining,hellendoorn2017deep,nguyen2013statistical}.

\paragraph{Existing Approaches}
Assessing the performance of different models and comparing them requires an accurate and reliable evaluation metric for the quality of their generated outputs.
The most common evaluation metrics are token-matching methods such as BLEU \citep{papineni2002bleu}, adopted from natural language processing (NLP), which are based on counting overlapping n-grams in the generated code and the reference code.
CrystalBLEU \citep{eghbali2022crystalbleu} extends BLEU by ignoring the counts of the 500 most occurring n-grams, arguing that they are trivially shared between the prediction and the reference. Nonetheless, both BLEU and CrystalBLEU rely on the lexical \emph{exact match} of tokens, which does not account for diversity in implementation, variable names, and code conventions. CodeBLEU \cite{ren2020codebleu} attempts to lower the requirement for lexical exact match, by relying on data-flow and Abstract Syntax Tree (AST) matching as well; nevertheless,  valid generations may have different ASTs and data-flow from the reference code, which may lead to low CodeBLEU score even when the prediction is correct. Further, \emph{partial} predictions may be useful for a programmer (for example, predicting the first line of a \texttt{for} loop, without the loop's body and closing), but accepting them may lead to partial code that does not parse, and thus cannot be evaluated by CodeBLEU.



Execution-based evaluation attempts to address these problems by running tests on the generated code to verify its functional correctness \cite{chen2021evaluating,athiwaratkun2022multi,li2022competition,wang2022execution,lai2022ds}. This provides a direct downstream measure of the functionality of the generated code, while being agnostic to diversity in implementation and style. However, execution-based evaluation requires datasets that are provided with hand-written test cases for each example, which is costly and labor-intensive to create. Further, executing model-generated code is susceptible to security threats,\footnote{\url{https://twitter.com/ludwig_stumpp/status/1619701277419794435?s=46&t=5vlJ05ph9UuGxQc17TXcrA}} and thus should be run in an isolated sandbox, which makes it technically cumbersome to work with iteratively.

\paragraph{Our Approach}
In this work, we introduce \cbs, an evaluation metric for code generation, leveraging pretrained models such as CodeBERT \citep{feng2020codebert}, and adopting best practices from natural language generation evaluation \citep{zhangbertscore}.
\cbs first encodes the generated code independently from the reference code, but with the natural language input instruction, if such exists; then, we compute the dot-product similarity between the encoded representations of each token in the generated code with each token in the reference code; finally, we take the best matching token vector pairs to compute \cbs$_{\mathrm{Precision}}$ and \cbs$_{\mathrm{Recall}}$. This allows \cbs to compare code pairs that are lexically different, while taking into account the (1) natural language instruction, if such provided; the (2) contextual information of each token, as encoded by the BERT-based model; and (3) implementation diversity, for example by giving a high similarity score to the encoding of \texttt{for} and the encoding of \texttt{while}. 

\paragraph{Example}
A concrete example is shown in \Cref{fig:intro_example}: given the reference code in \Cref{subfig:reference}, both BLEU and CodeBLEU prefer (rank higher) \emph{the non-equivalent} code in \Cref{subfig:noneq}, while our proposed \cbs prefers the code in \Cref{subfig:eq}, which \emph{is} functionally equivalent to the reference. We note that in this example, the variable names are identical across three code snippets. When the variable names of the reference are different than the variable names of the candidates, it is even much harder for token-matching approaches such as BLEU and CrystalBLEU to compare the reference with the candidates, while our \cbs can trivially match variable names according to their semantic similarity and their functional role in the code.
% Our approach is demonstrated in \Cref{fig:mainfigure}.

\paragraph{Evaluation}
We evaluate \cbs across multiple datasets, and we find that \cbs is \emph{more correlated with human preference and more correlated with functional correctness} than previous metrics. To evaluate human preference, we consider the CoNaLa dataset \citep{yin2018mining}, which is a dataset of 2879 pairs of Java Code and natural language context collected from StackOverflow. We compute the correlation between \cbs's score and  human preference scores that were collected by \citet{evtikhiev2022out} for the test set of CoNaLa. We use these human ratings to show that code that is preferred by humans is also ranked higher by \cbs than previous metrics such as BLEU \citep{papineni2002bleu}, CodeBLEU \citep{ren2020codebleu}, ROUGE, METEOR \citep{banerjee2005meteor}, chrF \citep{popovic2015chrF}, and CrystalBLEU \citep{eghbali2022crystalbleu}.

To evaluate the correlation between metric scores and functional correctness, we use the HumanEval dataset \citep{chen2021evaluating}, which consists of 165 programming problems along with input-output examples to test the generated solution. We compute the correlation between \cbs's score and whether the generated solution is functionally correct (according to the tests) and show that the code solutions that are functionally correct are also ranked higher by \cbs than previous metrics.

Finally, we show that the new meta-metric to evaluate different metrics called \emph{distinguishability}, which was proposed in the CrytstalBLEU paper \citep{eghbali2022crystalbleu}, can be easily manipulated since it compares \emph{absolute} scores between different metrics. The consequence of this is that while CrystalBLEU achieved a distinguishability score of 5.96, we can craft a variant of \cbs that achieves a distinguishability score of 10,000 (more than 1600 times higher!) by simple exponentiation of \cbs's output scalar. We thus argue that distinguishability is not a reliable meta-metric and is no substitute for execution-based- or human-rating when comparing different metrics.

\input{dl4c/intro_figure.tex}

\paragraph{Contributions} In summary, our main contributions are:
\begin{enumerate}
    \item The recognition of the absence of a reliable and static evaluation metric for code generation.
    \item A new metric for code similarity, which leverages the benefits of neural pretrained models, while not requiring any labeling or manually annotated data.
    \item An extensive evaluation across 4 programming languages, showing that \cbs is more correlated with human preference \emph{and} more correlated with execution correctness than all previous approaches including BLEU, CodeBLEU, and CrystalBLEU.
    \item While \cbs also achieves a higher ``Distinguishability''  than CrystalBLEU on the same datasets as CrystalBLEU, which proposed this meta-metric, we show that distinguishability can be easily manipulated and \cbs can achieve as high distinguishability as we wish, by simply exponentiating every output score. We thus suggest that distinguishability is not a reliable meta-metric in its current form, contrasting the findings of \citet{eghbali2022crystalbleu}.
    \item We pretrain and release 5 language-specific CodeBERT models to use with our publicly available code, for Java, Python, C, C++, and JavaScript. As of the time of this submission, our models were downloaded from the Huggingface Hub more than \textbf{25,000} times.
\end{enumerate}

==> fse/intro_code_example.tex <==
\newcommand{\lsize}{0.3015\textwidth}
\newcommand{\msize}{0.3015\textwidth}
\newcommand{\rsize}{0.385\textwidth}

\begin{figure*}[t]
\centering
\begin{minipage}{\lsize}
\centering
\textbf{Reference:} 
% Reference:
\end{minipage}
\begin{minipage}{\msize}
\centering
\textbf{Non-equivalent candidate:} 
% Non-equivalent implementation:
\end{minipage}
\begin{minipage}{\rsize}
\centering
\textbf{Equivalent candidate:} 
% Equivalent implementation:
\end{minipage} \\
\begin{minipage}{\lsize}
\begin{minted}[fontsize=\footnotesize,stripnl=false,framesep=1pt,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
int f(Object target) {
  int i = 0;
  for (Object elem: this.elements) {
    if (elem.equals(target)) {
      return i;
    }
    i++;
  }
  return -1;
}
\end{minted}
\end{minipage}
\begin{minipage}{\msize}
\begin{minted}[fontsize=\footnotesize,stripnl=false,framesep=1pt,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
boolean f(Object target) {
  for (Object elem: this.elements) {
    if (elem.equals(target)) {
      return true;
    }
  }
  |\\|
  return false;
}
|\\|

\end{minted}
\end{minipage}
\begin{minipage}{\rsize}
\begin{minted}[fontsize=\footnotesize,framesep=1pt,stripnl=false,frame=single,breaksymbolleft=\;,escapeinside=||]{java}
int f(Object target) {
  for (int i=0; i<this.elements.size(); i++) {
    Object elem = this.elements.get(i);
    if (elem.equals(target)) {
      return i;
    }
  }
  return -1;
}
|\\|
\end{minted}
\end{minipage}
\begin{minipage}{\lsize}
\centering
\begin{subfigure}[b]{1\linewidth}
% \vspace{2mm}
\caption{The ground truth reference}
% \caption{\phantom{\large{\textbf{Reference:} }}}
\label{subfig:reference}
\end{subfigure}
\end{minipage}
\begin{minipage}{\msize}
\centering
\begin{subfigure}[b]{1.05\linewidth}
\caption{\large{\textbf{\textcolor{red}{Preferred by BLEU \& CrystalBLEU}}}}
\label{subfig:noneq}
\end{subfigure}
\end{minipage}
\begin{minipage}{\rsize}
\centering
\begin{subfigure}[b]{1\linewidth}
\centering
\caption{\large{\textbf{\textcolor{ForestGreen}{Preferred by \cbs}}}}
\label{subfig:eq}
\end{subfigure}
\end{minipage}
\caption{An intuitive example for the usefulness of \cbs in measuring generated code: \Cref{subfig:reference} shows a reference code snippet in Java. This reference can be the ground truth code given as part of a test set. \Cref{subfig:noneq} and \Cref{subfig:eq} show two potential generated predictions.
%, with the main difference that \Cref{subfig:noneq} \emph{is not} functionally equivalent to the reference, while \Cref{subfig:eq} \emph{is} functionally equivalent to the reference. 
Among these two candidates and given the reference, both BLEU \citep{papineni2002bleu} and CrystalBLEU \citep{eghbali2022crystalbleu} prefer (score higher) the snippet in \Cref{subfig:noneq}, which \emph{is not} functionally equivalent to the reference, while our proposed \cbs prefers the code in \Cref{subfig:eq}, which \emph{is} functionally equivalent to the code in \Cref{subfig:reference}. 
}
\label{fig:intro_example}
\end{figure*}

==> fse/intro_figure.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fse/codebertscore.pdf}
\caption{A diagram illustrating \cbs: We use a language-specific CodeBERT model to encode each of $<$\emph{natural language}, \emph{reference code}$>$ and $<$\emph{natural language}, \emph{generated code}$>$. We then compute the pairwise cosine similarity between every encoded token in the reference and every encoded token in the generated code, ignoring the encoded context tokens and encoded punctuation tokens; finally, we take $max$ across the rows of the resulting matrix to compute \emph{Precision} (\textmd{\texttt{np.mean(np.max(similarity\_matrix, axis=0))}}), and the $max$ across columns to compute \emph{Recall} (\textmd{\texttt{np.mean(np.max(similarity\_matrix, axis=1))}}).
}
\label{fig:mainfigure}
\end{figure*}

==> humaneval_table_nostdev.tex <==
\begin{table*}[t]
    \centering
    % \resizebox{1\textwidth}{!}{ 
    \begin{tabular}{lcccccccc|cc}
    \toprule
     & \multicolumn{2}{c}{Java} & \multicolumn{2}{c}{C++} & \multicolumn{2}{c}{Python} & \multicolumn{2}{c}{JavaScript} & \multicolumn{2}{c}{Average}\\
    Metric & \ktt & \spp & \ktt & \spp & \ktt & \spp & \ktt & \spp & \ktt & \spp\\
    \midrule
    BLEU & .481 & .361 & .112 & .301 & .393 & .352 & .248 & .343&.308&.339 \\
    CodeBLEU & .496 & .324 & .175 & .201 & .366 & .326 & .261 & .299 &.325&.287 \\
    ROUGE-1 &  .516 & .318 & .262 & .260 & .368 & .334 & .279 & .280 &.356&.298 \\
    ROUGE-2 & .525 & .315 & .270 & .273 & .365 & .322 & .261 & .292&.355&.301 \\
    ROUGE-L & .508 & .344 & .258 & .288 & .338 & .350 & .271 & .293&.344&.319 \\
    METEOR & \textbf{.558} & \textbf{.383} & .301 & .321 & .418 & .402 & \textbf{.324} & \textbf{.415} & .400 & .380\\
    chrF & .532 & .319 & .319 & .321 & .394 & .379 & .302 & .374 &.387&.348 \\
    CrystalBLEU & .471 & .273 & .046 & .095 & .391 & .309 & .118 & .059 &.257&.184 \\
    \midrule
    \cbs & \textbf{.553} & .369 & \textbf{.327} & \textbf{.393} & \textbf{.422} & \textbf{.415} & \textbf{.319} & .402 & \textbf{.405} & \textbf{.395}\\
    \bottomrule
    \end{tabular}
    % }
    \caption{The \kt (\ktt) and \spe (\spp) correlations of each metric with the functional correctness %(zeros means incorrect and one means correct) of a program 
    on \he in multiple languages. %-Java, C++, Python and JavaScript.
    % The best performance is in \textbf{bold}. 
    The correlation coefficients are reported as the average across three runs. Standard deviation is shown in \Cref{tab:corr_func_appendix} due to space limitations.}
    \label{tab:corr_func}
\end{table*}
